A Renyi Quantum Null Energy Condition: Proof for Free Field Theories

The Quantum Null Energy Condition (QNEC) is a lower bound on the stress-energy tensor in quantum field theory that has been proved quite generally. It can equivalently be phrased as a positivity condition on the second null shape derivative of the relative entropy $S_{\text{rel}}(\rho||\sigma)$ of an arbitrary state $\rho$ with respect to the vacuum $\sigma$. The relative entropy has a natural one-parameter family generalization, the Sandwiched Renyi divergence $S_n(\rho||\sigma)$, which also measures the distinguishability of two states for arbitrary $n\in[1/2,\infty)$. A Renyi QNEC, a positivity condition on the second null shape derivative of $S_n(\rho||\sigma)$, was conjectured in previous work. In this work, we study the Renyi QNEC for free and superrenormalizable field theories in spacetime dimension $d>2$ using the technique of null quantization. In the above setting, we prove the Renyi QNEC in the case $n>1$ for arbitrary states. We also provide counterexamples to the Renyi QNEC for $n<1$.

==> deleted-sections.tex <==
\subsection{Sandwiched Renyi divergence}

Let $\mathcal{A}$ be an algebra of operators associated with some region $A$ of the spacetime. Consider a state $\ket{\Psi}$ (not necessarily the vacuum state) which is cyclic and separating for both $\mathcal{A}$ and its commutant $\mathcal{A}'$. The state $\ket{\Psi}$ is cyclic and separating for algebra $\mathcal{A}$ if for $\OO_{A}\in\mathcal{A}$, $\mathcal{O}_{A}\ket{\Psi}$ is dense in the Hilbert space and $\OO_{A}\ket{\Psi} \, = \, 0$ implies $\OO_{A}=0$ respectively [CITATION]. The Tomita Takesaki operator $S_{\psi}$ for state $\ket{\Psi}$ is defined as [CITE]
\begin{align}
    S_{\psi} \, \OO_{A}\ket{\Psi} \, \equiv \, \OO^{\dagger}_{A} \ket{\Psi} \, ,%\quad\quad \OO_{A} \in \mathcal{A} \, .
\end{align}
for all $\OO_{A} \in \mathcal{A}$. The modular Hamiltonian $\Delta_{\psi}$ for state $\ket{\Psi}$ is then defined as
\begin{align}
    \Delta_{\psi} \, \equiv \, S^{\dagger}_{\psi} \, S_{\psi} \, .
\end{align}
From this definition, we note that $\Delta_{\psi}$ is Hermitian and positive-definite operator. Moreover, we note that this operator leaves the state $\ket{\Psi}$ invariant:
\begin{align}
    \Delta_{\psi}\ket{\Psi} \, = \, \ket{\Psi} \, .
\end{align}

In quantum field theory, the operators $S_{\psi}$ and $\Delta_{\psi}$ are unbounded operator [CITE]. This means that $\Delta_{\psi}\ket{\Lambda}$ may not have a finite norm and hence, it may not be a well-defined state. In fact, for dense states of the form $\OO_{A}\ket{\Psi}$ where $\OO_{A}\in\mathcal{A}$, $\Delta^{\alpha}_{\psi} \, \OO_{A}\ket{\Psi}$ has finite norm only for $O \le \alpha \le 1/2$ [CITE]. We will use this fact later in this section to determine for which states the sandwiched Renyi divergence is not divergent.

The relative entropy and Renyi divergences between two states is defined in terms of the relative modular Hamiltonian which we now review. 

\subsection{Modular Fourier Space} \label{sec-mod-freq-sp} 

Consider a state $\ket{\Psi}$ (not necessarily the vacuum state) which is cyclic and separating for subalgebra $\mathcal{A}$ and its commutant $\mathcal{A}'$. Let $\Delta_{\Psi}$ be the modular operator of this state. Given a local operator $\OO \in \mathcal{A}$, the `modular-flowed' operator defined as \cite{} %, $A_{s}$ is also in $\mathcal{A}$. That is,
\begin{align}
    \OO_{s} \, \equiv \, \Delta_{\psi}^{-is/2\pi} \, \OO \, \Delta_{\psi}^{is/2\pi} \, 
\end{align}
is also in $\mathcal{A}$. Unless in some special cases, $\OO_{s}$ is a non-local operator. This is why it is instructive to write the flowed operator in the `modular frequency' space which was introduced in \cite{Faulkner:2017vdd}:
\begin{align}
    \OO_{\omega} \, \equiv \, \frac{1}{2\pi} \, \int_{-\infty}^{\infty} ds \, e^{-is\omega} \, \Delta_{\psi}^{-is/2\pi} \, \OO \, \Delta_{\psi}^{is/2\pi} \, . \label{eq-def-Aw-TT}
\end{align}
This mode decomposition proved to be an important ingredient in the boundary reconstruction of a bulk operator in the entanglement wedge \cite{Faulkner:2017vdd}. 

In this work we assume that, in the presence of some suitable UV cutoff, the Hilbert space factorizes into the Hilbert space of subregions $A$ and $A'$ of a cauchy slice: $\mathcal{H} \, = \, \mathcal{H}_{A}\otimes\mathcal{H}_{A'} \, $. We take $\mathcal{A}$ and $\mathcal{A}'$ to be the algebra of operators acting on $\mathcal{H}_{A}$ and $\mathcal{H}_{A'}$ respectively. In this case, the modular operator $\Delta_{\psi}$ can be written as
\begin{align}
    \Delta_{\Psi} \, = \, \rho \otimes (\rho')^{-1} \, , \label{eq-Delta-mat}
\end{align}
where $\rho$ and $\rho'$ are the reduced states defined as
\begin{align}
    \rho \, \equiv \, \text{tr}_{A'} \, \ket{\psi}\bra{\psi} \, \quad\quad\quad \, \rho' \, \equiv \, \text{tr}_{A} \, \ket{\psi}\bra{\psi} \, .
\end{align}
In terms of the density matrices, the operator $\OO_{\omega}$ in Eq.~\eqref{eq-def-Aw-TT} simplifies to %A local operator in the   
\begin{align}
    \OO_{\omega} \, \equiv \, \frac{1}{2\pi} \, \int_{-\infty}^{\infty} ds \, e^{-is\omega} \, \rho^{-is/2\pi} \, \OO \, \rho^{is/2\pi} \, . \label{eq-def-Aw}
\end{align}
This decomposition of an operator into modular frequency modes was used used in \cite{May:2018tir} to write the Renyi relative entropy as a correlation function. Inspired by this, we will use this decomposition to write the shape deformation of the Renyi relative entropies as correlation functions. 

We now discuss some properties of the operators in the Modular frequency space that we will use in the later sections. Note the completeness relation
\begin{align}
    \OO \, = \, \int_{-\infty}^{\infty} d\omega \, \OO_{\omega} \, .\label{eq-Aw-comp}
\end{align}
Now consider a basis in which $\rho$ is diagonal. That is,
\begin{align}
    \rho \, \ket{\kappa} \, = \, e^{-2\pi\kappa} \, \ket{\kappa} \, .
\end{align}
In this basis, the matrix elements of $\OO_{\omega}$ have a simple form:
\begin{align}
    \bra{\kappa} \OO_{\omega} \ket{\kappa'} \, = \, \delta\Big(\omega - \big(\kappa-\kappa'\big)\Big) \,\, \bra{\kappa}  \OO \ket{\kappa'} \, . \label{eq-Aw-mat}
\end{align}
This means that for any arbitrary function $h(x)$, we get
\begin{align}
    h(\kappa-\kappa') \, \bra{\kappa} \OO \ket{\kappa'} \, = \, \int_{-\infty}^{\infty} d\omega \, h(\omega) \, \bra{\kappa} \OO_{\omega} \ket{\kappa'} \, . \label{eq-A-mat-h}
\end{align}
Finally, note the commutation relation
\begin{align}
    \rho \, A_{\omega} \,  = \, e^{-2\pi\omega} \, A_{\omega} \, \rho \, . \label{eq-Aw-commutation}
\end{align}
In addition to these, the operators $\OO_{\omega}$ has many other interesting properties. For example, their correlation functions satisfy various KMS conditions \cite{Faulkner:2017vdd}. We will not be using those properties in this work. 

\subsection{Sandwiched state on a null plane} \label{sec-null-sand-st}

As discussed in the last subsection, we only need to consider the $O(\mathcal{A})$ contribution to the SRRE to check if the Renyi QNEC conjecture in Eq.~\eqref{eq-null-qnec-conj} is correct. The perturbative calculation of relative entropy and Renyi relative entropy has been performed extensively in the past \cite{Faulkner:2014jva,Lashkari:2015hha,Faulkner:2017tkh,May:2018tir,Ugajin:2018rwd,Bao:2019aol}. However, all these perturbative analysis are only valid for two `nearby' states. This assumption is not valid in our case since the state $\rho^{(0)}$ in Eq.~\eqref{eq-null-state-0} is not the vacuum state unless $\rho_{\aux}^{(0)} \, = \, \sigma_{\aux}$. Therefore, we can not simply use the known perturbative results and will have to derive an expression for $Z_{n}^{(1,1)}$. 

Note that the perturbative state in Eq.~\eqref{eq-null-state-1-int} is ambiguous because $\{\ket{\alpha}\}$ is an arbitrary basis for the auxiliary system. In this section, we will fix this choice. Our choice is motivated by the fact that this will simplify the derivation of $Z_{n}^{(1,1)}$.

Consider the (unnormalized) sandwiched state
\begin{align}
    \tilde{\rho}(\lambda) \, \equiv \, \left(\sigma^{\frac{1-n}{2n}} \, \rho(\lambda) \, \sigma^{\frac{1-n}{2n}}\right)^{n} \, . \label{eq-null-sand-st}
\end{align}
(Note that $\trho$ explicitly depend on $n$ though we are not denoting this $n$ dependence to keep the notations cleaner.) Now using Eq.~\eqref{eq-null-state}, we get%We can expand $\trho$ as in Eq.~\eqref{eq-null-state}:
\begin{align}
        \big(\trho(\lambda)\big)^{1/n} \, = \, \sigma^{\frac{1-n}{2n}} \, \rho^{(0)} \, \sigma^{\frac{1-n}{2n}} \, + \, \mathcal{A}^{1/2} \, \sigma^{\frac{1-n}{2n}} \, \rho^{(1)}(\lambda) \, \sigma^{\frac{1-n}{2n}} \, + \, O(\mathcal{A}) \, . \label{eq-null-sand-exp}
\end{align}
Using Eq.~\eqref{eq-null-vac} and Eq.~\eqref{eq-null-state-0}, we find that the order $O(\mathcal{A}^{0})$ term is given by
\begin{align}
    \sigma^{\frac{1-n}{2n}} \, \rho^{(0)} \, \sigma^{\frac{1-n}{2n}} \, =& \,\, \sigma_{p}^{1/n} \otimes \left( \sigma_{\aux}^{\frac{1-n}{2n}} \, \rho_{\aux}^{(0)} \, \sigma_{\aux}^{\frac{1-n}{2n}} \right) \, \nonumber\\
    =& \,\, \left( \sigma_{p} \otimes \trho_{\aux}^{(0)} \right)^{1/n} \, ,
\end{align}
where we have defined similarly to Eq.~\eqref{eq-null-sand-st}
\begin{align}
    \trho_{\aux}^{(0)} \, \equiv \, \left( \sigma_{\aux}^{\frac{1-n}{2n}} \, \rho_{\aux}^{(0)} \, \sigma_{\aux}^{\frac{1-n}{2n}} \right)^{n} \, .
\end{align}
Now let us consider the order $O(\mathcal{A}^{1/2})$ term in Eq.~\eqref{eq-null-sand-exp}. Using Eq.~\eqref{eq-null-vac} and Eq.~\eqref{eq-null-state-1-int}, we get
\begin{align}
    \sigma^{\frac{1-n}{2n}} \, \rho^{(1)}(\lambda) \, \sigma^{\frac{1-n}{2n}} \, = \, \sum_{\alpha\beta} \, &\left( \sigma_{p}^{\frac{1-n}{2n}} \cdot \sigma_{p} \, \int dr d\theta \, f_{\alpha\beta}(r,\theta) \, \partial\Phi(r e^{i\theta} \, - \, \lambda) \, \cdot \sigma_{p}^{\frac{1-n}{2n}} \right) \, \nonumber\\ \otimes& \, \left(\sigma_{\aux}^{\frac{1-n}{2n}}\ket{\alpha}\bra{\beta}\sigma_{\aux}^{\frac{1-n}{2n}}\right) \, .
\end{align}
Adding complete sets of basis, we write this as
\begin{align}
    \sigma^{\frac{1-n}{2n}} \, \rho^{(1)}(\lambda) \, \sigma^{\frac{1-n}{2n}} \, = \, \sum_{\alpha'\beta'}\sum_{\alpha\beta} \, &\left( \sigma_{p}^{\frac{1-n}{2n}} \cdot \sigma_{p} \, \int dr d\theta \, f_{\alpha\beta}(r,\theta) \, \partial\Phi(r e^{i\theta} \, - \, \lambda) \, \cdot \sigma_{p}^{\frac{1-n}{2n}} \right) \, \nonumber\\ \otimes& \, \left(\bra{\alpha'}\sigma_{\aux}^{\frac{1-n}{2n}}\ket{\alpha} \bra{\beta}\sigma_{\aux}^{\frac{1-n}{2n}} \ket{\beta'} \, \cdot \, \ket{\alpha'}\bra{\beta'} \right) \, . %\label{eq-null-sand-1-int}
\end{align}
We now define 
\begin{align}
    \tf_{\alpha\beta}(r,\theta) \, \equiv \, \sum_{\alpha'\beta'} \, f_{\alpha'\beta'}(r,\theta) \, \bra{\alpha}\sigma_{\aux}^{\frac{1-n}{2n}}\ket{\alpha'} \, \bra{\beta'}\sigma_{\aux}^{\frac{1-n}{2n}} \ket{\beta} \, . 
\end{align}
It is not hard to check that $\tf_{\alpha\beta}$ satisfies the reality condition in Eq.~\eqref{eq-null-reality-1}:
\begin{align}
    \tf_{\alpha\beta}(r,2\pi-\theta) \, = \, \tf_{\beta\alpha}^{*}(r,\theta) \, .% \label{eq-null-reality}
\end{align}
With this definition, we simplify Eq.~\eqref{eq-null-sand-1-int} to get
\begin{align}
    \sigma^{\frac{1-n}{2n}} \, \rho^{(1)}(\lambda) \, \sigma^{\frac{1-n}{2n}} \, = \, \sum_{\alpha\beta}  \left( \sigma_{p}^{\frac{1-n}{2n}} \cdot \sigma_{p} \, \int dr d\theta \, \tf_{\alpha\beta}(r,\theta) \, \partial\Phi(r e^{i\theta}  -  \lambda) \, \cdot \sigma_{p}^{\frac{1-n}{2n}} \right) \, \otimes \, \ket{\alpha}\bra{\beta}  \, . %\label{eq-null-sand-1-int-2}
\end{align}
So far we have not fixed the choice of the basis $\{\ket{\alpha}\}$. Now we take $\{\ket{\alpha}\}$ to be the basis in which $\trho^{(0)}_{\aux}$ is diagonal:
\begin{align}
    \trho^{(0)}_{\aux} \, \ket{\alpha} \, = \, e^{-2\pi K_{\alpha}} \, \ket{\alpha} \, ,  \label{eq-null-trho-eigen}
\end{align}
Now we follow \cite{Bousso:2015wca} and define:
\begin{align}
    E_{\alpha\beta}(\theta) \, \equiv \, e^{\theta(K_{\alpha}-K_{\beta})} \, \ket{\alpha}\bra{\beta} \, . %\label{eq-null-def-Eab}
\end{align}
With this, we get
\begin{align}
   \left(\trho_{\aux}^{(0)}\right)^{\frac{1-n}{2n}} \, \trho_{\aux}^{(0)} \, E_{\alpha\beta}(\theta) \, \left(\trho_{\aux}^{(0)}\right)^{\frac{1-n}{2n}} \, = \, e^{-(2\pi-\theta)K_{\alpha}} \, e^{-\theta K_{\beta}} \, \, e^{ \frac{\pi(n-1)}{n} (K_{\alpha}+K_{\beta})} \,  \ket{\alpha}\bra{\beta} \, .
\end{align}
Now note that $\tf_{\alpha\beta}(r,\theta)$ is arbitrary as long as it satisfies the reality condition in Eq.~\eqref{eq-null-reality}. This means we can rescale $\tf_{\alpha\beta}(r,\theta)$ by
\begin{align}
    \tf_{\alpha\beta}(r,\theta) \, \longrightarrow \, e^{(2\pi-\theta)K_{\alpha}} \, e^{\theta K_{\beta}} \, \, e^{ \frac{\pi(1-n)}{n} (K_{\alpha}+K_{\beta})} \, \tf_{\alpha\beta}(r,\theta) \, .
\end{align}
It is not difficult to see that the rescaled $\tf_{\alpha\beta}(r,\theta)$ also satisfies Eq.~\eqref{eq-null-reality}.  Now we can write Eq.~\eqref{eq-null-sand-1-int-2} as
\begin{align}
    \sigma^{\frac{1-n}{2n}} \, \rho^{(1)}(\lambda) \, \sigma^{\frac{1-n}{2n}} \, = \, \sum_{\alpha\beta} \, &\left( \sigma_{p}^{\frac{1-n}{2n}} \cdot \sigma_{p} \, \int dr d\theta \, \tf_{\alpha\beta}(r,\theta) \, \partial\Phi(r e^{i\theta} \, - \, \lambda) \, \cdot \sigma_{p}^{\frac{1-n}{2n}} \right) \, \nonumber\\ \otimes& \, \left( \left(\trho_{\aux}^{(0)}\right)^{\frac{1-n}{2n}} \, \cdot \, \trho_{\aux}^{(0)} \, E_{\alpha\beta}(\theta) \, \cdot \,  \left(\trho_{\aux}^{(0)}\right)^{\frac{1-n}{2n}} \right) \, . %\label{eq-null-sand-1-int-3}
\end{align}
To simplify this result, we define analogous to Eq.~\eqref{eq-null-state-0} and Eq.~\eqref{eq-null-state-1-int}:
\begin{align}
    \trho^{(0)} \, = \, \sigma_{p} \, \otimes \, \trho^{(0)}_{\aux} \, , %\label{eq-null-sand-0}
\end{align}
and 
\begin{align}
    \trho^{(1)}(\lambda)  \, = \, \sum_{\alpha\beta} \, \trho^{(0)} \, \int dr d\theta \, \tf_{\alpha\beta}(r,\theta) \, \left( \partial\Phi(r e^{i\theta} \, - \, \lambda) \,  \otimes \, E_{\alpha\beta}(\theta) \right) \, . \label{eq-null-state-1-fin}
\end{align}
In terms of these, we simplify Eq.~\eqref{eq-null-sand-1-int-3} to get
\begin{align}
    \sigma^{\frac{1-n}{2n}} \, \rho^{(1)}(\lambda) \, \sigma^{\frac{1-n}{2n}} \, = \, \left(\trho^{(0)}\right)^{\frac{1-n}{2n}} \cdot \, \trho^{(1)}(\lambda) \, \cdot \, \left(\trho^{(0)}\right)^{\frac{1-n}{2n}} \, .
\end{align}

To summarize, we have found that we can write the expansion of the sandwiched state in Eq.~\eqref{eq-null-sand-exp} as
\begin{align}
     \big(\trho(\lambda)\big)^{1/n} \, = \, \big(\trho^{(0)} \big)^{1/n} \, + \, \mathcal{A}^{1/2} \, \left(\trho^{(0)}\right)^{\frac{1-n}{2n}} \cdot \, \trho^{(1)}(\lambda) \, \cdot \, \left(\trho^{(0)}\right)^{\frac{1-n}{2n}} \, + \, O(\mathcal{A}) \, . \label{eq-null-sand-exp-final}
\end{align}
This perturbative expansion together with Eq.~\eqref{eq-null-sand-0} and Eq.~\eqref{eq-null-state-1-fin} are the main results of this section. 


\subsection{$Z_{n}^{(1,1)}$ as correlation functions} \label{sec-null-zn-corr}

In this subsection, our goal is to derive an expression for $Z_{n}^{(1,1)}$ that we can later use to check if Renyi QNEC in Eq.~\eqref{eq-null-renyi-qnec} is true. We start with Eq.~\eqref{eq-null-zn-eqv} that we derived in the last subsection:
%Recall from Eq.~\eqref{eq-null-hatz-def} and Eq.~\eqref{eq-null-z-def} that
%\begin{align}
%    Z_{n}(\lambda) \, =& \,\, \frac{1}{n-1} \, \tr \, \left(\sigma^{\frac{1-n}{2n}} \, \rho(\lambda) \, \sigma^{\frac{1-n}{2n}}\right)^{n} \, , \\
%    =& \,\, \frac{1}{n-1} \, \tr \, \trho(\lambda) \, ,
%\end{align}
%where we have used Eq.~\eqref{eq-null-sand-st}. Now using Eq.~\eqref{eq-null-sand-exp-final}, we get
\begin{align}
    Z_{n}(\lambda) \, = \, \frac{1}{n-1} \, \tr \, \Bigg( \big(\trho^{(0)} \big)^{1/n} \, + \, \mathcal{A}^{1/2} \, \left(\trho^{(0)}\right)^{\frac{1-n}{2n}} \cdot \, \trho^{(1)}(\lambda) \, \cdot \, \left(\trho^{(0)}\right)^{\frac{1-n}{2n}} \Bigg)^{n} \, .
\end{align}
Recall that for integer $n$, we have
\begin{align}
    \tr \left(A_{0} + A_{1} \right)^{n} \, = \, \tr A_{0}^{n} \, + \, n \, \tr \left(A_{0}^{n-1} \, A_{1} \right) \, + \, \frac{n}{2} \, \sum_{k=0}^{n-2} \, \tr \left(A_{0}^{k} \, A_{1} \, A_{0}^{n-2-k} \, A_{1} \right) \, + \, ... \, .
\end{align}
Using this identity, we deduce that (for integer $n$):
\begin{align}
    Z_{n}^{(1,1)}(\lambda) \, = \, \frac{n}{2(n-1)} \, \sum_{k=1}^{n-1} \, \tr \left( \left(\trho^{(0)}\right)^{-1+\frac{k}{n}}  \, \trho^{(1)}(\lambda) \, \left(\trho^{(0)}\right)^{-\frac{k}{n}}  \, \trho^{(1)}(\lambda) \, \right) \, . \label{eq-null-z11-int}
\end{align}
Now we evaluate the trace in a basis in which $\trho^{(0)}$ is diagonal:
\begin{align}
    \trho^{(0)} \, \ket{\kappa} \, = \, e^{-2\pi \kappa} \, \ket{\kappa} \, .
\end{align}
%The eigenvalues $\kappa$ are related to the eigenvalues $K_{\alpha}$ of $\trho^{(0)}_{\aux}$, but this relation is not important in our analysis. 
In this basis, the trace in Eq.~\eqref{eq-null-z11-int} becomes
\begin{align}
    Z_{n}^{(1,1)}(\lambda) \, =& \, \frac{n}{2(n-1)} \, \int d\kappa \int d\kappa' \,\, \sum_{k=1}^{n-1} \, e^{2\pi\kappa} \, e^{-2\pi(\kappa-\kappa')\frac{k}{n}} \, \left|\bra{\kappa}\trho^{(1)}(\lambda)\ket{\kappa'}\right|^{2} \, ,\\
    =& \, - \, \frac{n}{2(n-1)} \, \int d\kappa \int d\kappa' \,\,   \frac{e^{2\pi \left(\frac{n-1}{n}\right) \kappa}  - e^{2\pi \left(\frac{n-1}{n}\right) \kappa'}}{e^{-2\pi \kappa/n}  - e^{-2\pi \kappa'/n}} \, \left|\bra{\kappa}\trho^{(1)}(\lambda)\ket{\kappa'}\right|^{2} \, .  \label{eq-null-z11-int-2}
\end{align}
Note that even though Eq.~\eqref{eq-null-z11-int-2} was derived by assuming $n$ is an integer, the result is valid for all $n$. This can be derived using the matrix identities in Appendix \ref{sec-app-iden}. See \cite{May:2018tir} for details. 

We now take the derivative of Eq.~\eqref{eq-null-z11-int-2} to get
\begin{align}
    \ddot{Z}_{n}^{(1,1)}(\lambda) \, = \, - &\, \frac{n}{(n-1)} \, \int d\kappa \int d\kappa' \,\,   \frac{e^{2\pi \left(\frac{n-1}{n}\right) \kappa}  - e^{2\pi \left(\frac{n-1}{n}\right) \kappa'}}{e^{-2\pi \kappa/n}  - e^{-2\pi \kappa'/n}} \, \nonumber\\
    \times & \left(\bra{\kappa}{\trho}^{(1)}(\lambda)\ket{\kappa'}\bra{\kappa'}\ddot{\trho}^{(1)}(\lambda)\ket{\kappa}+\bra{\kappa}\dot{\trho}^{(1)}(\lambda)\ket{\kappa'}\bra{\kappa'}\dot{\trho}^{(1)}(\lambda)\ket{\kappa}\right) \, ,\label{eq-null-z11-dd-int}
\end{align}
where dot represent derivative with respect to $\lambda$. 

Now using Eq.~\eqref{eq-null-state-1-fin}, we get
\begin{align}
    \trho^{(1)}(\lambda = 0)  \, = \, \sum_{\alpha\beta} \, \int dr d\theta \, \tf_{\alpha\beta}(r,\theta) \, \trho^{(0)} \OO^{\alpha\beta}(r,\theta) \, ,%\left( \partial\Phi(r e^{i\theta} \, - \, \lambda) \,  \otimes \, E_{\alpha\beta}(\theta) \right) \, .
\end{align}
where
\begin{align}
    \OO^{\alpha\beta}(r,\theta) \, \equiv \, \partial\Phi(re^{i\theta}) \, \otimes \, E_{\alpha\beta}(\theta) \, .\label{eq-OO-0}
\end{align}
Similarly, we write 
\begin{align}
    \dot{\trho}^{(1)}(\lambda = 0)  \, =& \, - \, \sum_{\alpha\beta} \, \int dr d\theta \, \tf_{\alpha\beta}(r,\theta) \, \trho^{(0)} \dot{\OO}^{\alpha\beta}(r,\theta) \, ,\\
    \ddot{\trho}^{(1)}(\lambda = 0)  \, =& \,  \sum_{\alpha\beta} \, \int dr d\theta \, \tf_{\alpha\beta}(r,\theta) \, \trho^{(0)} \ddot{\OO}^{\alpha\beta}(r,\theta) \, ,
    %\left( \partial\Phi(r e^{i\theta} \, - \, \lambda) \,  \otimes \, E_{\alpha\beta}(\theta) \right) \, .
\end{align}
where
\begin{align}
    \dot{\OO}^{\alpha\beta}(r,\theta) \, &\equiv \, \partial^{2}\Phi(re^{i\theta}) \, \otimes \, E_{\alpha\beta}(\theta) \, ,\label{eq-dOO-0}\\
    \ddot{\OO}^{\alpha\beta}(r,\theta) \, &\equiv \, \partial^{3}\Phi(re^{i\theta}) \, \otimes \, E_{\alpha\beta}(\theta) \, . \label{eq-ddOO-0}
\end{align}

In terms of these operators, Eq.~\eqref{eq-null-z11-dd-int} becomes
\begin{align}
\ddot{Z}_{n}^{(1,1)}(\lambda=0) \, = \, - &\, \frac{n}{(n-1)} \, \int d\kappa \int d\kappa' \,\,   \frac{e^{2\pi \left(\frac{n-1}{n}\right) \kappa}  - e^{2\pi \left(\frac{n-1}{n}\right) \kappa'}}{e^{-2\pi \kappa/n}  - e^{-2\pi \kappa'/n}} \, e^{-2\pi (\kappa+ \kappa')} \nonumber\\
&\times \, \sum_{\alpha'\beta'}\sum_{\alpha\beta} \, \int dr_{1}dr_{2} \, \int_{0}^{2\pi} d\theta_{1}d\theta_{2} \,\, \tf_{\alpha\beta}(r_{1},\theta_{1}) \, \tf_{\alpha'\beta'}(r_{2},\theta_{2}) \nonumber\\
&\times \, \Big(\bra{\kappa}{\OO}^{\alpha\beta}(r_{1},\theta_{1})\ket{\kappa'}\bra{\kappa'}\ddot{\OO}^{\alpha'\beta'}(r_{2},\theta_{2})\ket{\kappa} \nonumber\\ & \quad + \, \bra{\kappa}\dot{\OO}^{\alpha\beta}(r_{1},\theta_{1})\ket{\kappa'}\bra{\kappa'}\dot{\OO}^{\alpha'\beta'}(r_{2},\theta_{2})\ket{\kappa}\Big) \, . \label{eq-null-z11-dd-int-2}
\end{align}
To simplify this result, we define
\begin{align}
    F_{n}(x) \, = \, \frac{n}{1-n} \, \frac{e^{2\pi \left(\frac{n-1}{n}\right) x}  - 1}{e^{-2\pi x/n}  - 1} \, . \label{eq-null-Fn-def}
\end{align}
With this, Eq.~\eqref{eq-null-z11-dd-int-2} becomes
\begin{align}
    \ddot{Z}_{n}^{(1,1)} \, = \, \sum_{\alpha'\beta'}\sum_{\alpha\beta} \, &\int dr_{1}dr_{2} \, \int_{0}^{2\pi} d\theta_{1}d\theta_{2} \,\, \tf_{\alpha\beta}(r_{1},\theta_{1}) \, \tf_{\alpha'\beta'}(r_{2},\theta_{2}) \int d\kappa \int d\kappa' \, \nonumber\\ \times\, & F_{n}(\kappa-\kappa') \, e^{-2\pi\kappa} \, \Big(\bra{\kappa}{\OO}^{\alpha\beta}(r_{1},\theta_{1})\ket{\kappa'}\bra{\kappa'}\ddot{\OO}^{\alpha'\beta'}(r_{2},\theta_{2})\ket{\kappa} \nonumber\\ & \quad\quad\quad\quad\quad + \, \bra{\kappa}\dot{\OO}^{\alpha\beta}(r_{1},\theta_{1})\ket{\kappa'}\bra{\kappa'}\dot{\OO}^{\alpha'\beta'}(r_{2},\theta_{2})\ket{\kappa}\Big) \, . \label{eq-null-z11-dd-int-3}
\end{align}

We need to write Eq.~\eqref{eq-null-z11-dd-int-3} as a trace which we can then later write as a correlation functions. To do this, we follow \cite{May:2018tir} and write a local operator in the   `modular frequency' space which was introduced in \cite{Faulkner:2017vdd}:
\begin{align}
    \OO_{\omega} \, \equiv \, \frac{1}{2\pi} \, \int_{-\infty}^{\infty} ds \, e^{-is\omega} \, \big( \trho^{(0)} \big)^{-is/2\pi} \, \OO \, \big( \trho^{(0)} \big)^{is/2\pi} \, . \label{eq-null-def-0w}
\end{align}
Let us list some properties of the operators in the Modular frequency space. First, note that 
\begin{align}
    \OO \, = \, \int_{-\infty}^{\infty} d\omega \, \OO_{\omega} \, .\label{eq-null-OOw-comp}
\end{align}
Secondly, note that 
\begin{align}
    \bra{\kappa} \OO_{\omega} \ket{\kappa'} \, = \, \delta\Big(\omega - \big(\kappa-\kappa'\big)\Big) \,\, \bra{\kappa}  \OO \ket{\kappa'} \, . \label{eq-null-OOw-mat}
\end{align}
Finally, note the commutation relation
\begin{align}
    \trho^{(0)} \, \OO_{\omega} \,  = \, e^{-2\pi\omega} \, \OO_{\omega} \, \trho^{(0)} \, . \label{eq-null-OOw-commutation}
\end{align}
Now we will use these three properties to write Eq.~\eqref{eq-null-z11-dd-int-3} as a correlation function. We start by using Eq.~\eqref{eq-null-OOw-comp} to write Eq.~\eqref{eq-null-z11-dd-int-3} as
\begin{align}
    \ddot{Z}_{n}^{(1,1)} \, = \, &\sum_{\alpha'\beta'}\sum_{\alpha\beta} \, \int dr_{1}dr_{2} \, \int_{0}^{2\pi} d\theta_{1}d\theta_{2} \,\, \tf_{\alpha\beta}(r_{1},\theta_{1}) \, \tf_{\alpha'\beta'}(r_{2},\theta_{2}) \, \int_{-\infty}^{\infty} d\omega \,  \nonumber\\ \times\, & \int d\kappa \int d\kappa' \, F_{n}(\kappa-\kappa') \, e^{-2\pi\kappa} \, \Big(\bra{\kappa}{\OO}_{\omega}^{\alpha\beta}(r_{1},\theta_{1})\ket{\kappa'}\bra{\kappa'}\ddot{\OO}^{\alpha'\beta'}(r_{2},\theta_{2})\ket{\kappa} \nonumber\\ & \quad\quad\quad\quad\quad\quad\quad + \, \bra{\kappa}\dot{\OO}_{\omega}^{\alpha\beta}(r_{1},\theta_{1})\ket{\kappa'}\bra{\kappa'}\dot{\OO}^{\alpha'\beta'}(r_{2},\theta_{2})\ket{\kappa}\Big) \, . \label{eq-null-z11-dd-int-4}
\end{align}
Now using Eq.~\eqref{eq-null-OOw-mat}, we write the above result as
\begin{align}
    \ddot{Z}_{n}^{(1,1)} \, = \, &\sum_{\alpha'\beta'}\sum_{\alpha\beta} \, \int dr_{1}dr_{2} \, \int_{0}^{2\pi} d\theta_{1}d\theta_{2} \,\, \tf_{\alpha\beta}(r_{1},\theta_{1}) \, \tf_{\alpha'\beta'}(r_{2},\theta_{2}) \, \int_{-\infty}^{\infty} d\omega \, F_{n}(\omega)  \nonumber\\ \times\, & \int d\kappa \int d\kappa' \,  \, e^{-2\pi\kappa} \, \Big(\bra{\kappa}{\OO}_{\omega}^{\alpha\beta}(r_{1},\theta_{1})\ket{\kappa'}\bra{\kappa'}\ddot{\OO}^{\alpha'\beta'}(r_{2},\theta_{2})\ket{\kappa} \nonumber\\ & \quad\quad\quad\quad\quad\quad\quad + \, \bra{\kappa}\dot{\OO}_{\omega}^{\alpha\beta}(r_{1},\theta_{1})\ket{\kappa'}\bra{\kappa'}\dot{\OO}^{\alpha'\beta'}(r_{2},\theta_{2})\ket{\kappa}\Big) \, .\label{eq-null-z11-dd-int-5}
\end{align}
Equivalently, we can write this as
\begin{align}
    \ddot{Z}_{n}^{(1,1)}& \, = \,\,  \sum_{\alpha'\beta'}\sum_{\alpha\beta} \, \int dr_{1}dr_{2} \, \int_{0}^{2\pi} d\theta_{1}d\theta_{2} \,\, \tf_{\alpha\beta}(r_{1},\theta_{1}) \, \tf_{\alpha'\beta'}(r_{2},\theta_{2}) \,\,  \int_{-\infty}^{\infty} d\omega \, F_{n}(\omega) \nonumber\\ &\times  
    \Bigg( \tr \Big( \trho^{(0)} \, {\OO}_{\omega}^{\alpha\beta}(r_{1},\theta_{1}) \, \ddot{\OO}^{\alpha'\beta'}(r_{2},\theta_{2})\Big) + \, \tr \Big( \trho^{(0)} \, \dot{\OO}_{\omega}^{\alpha\beta}(r_{1},\theta_{1}) \, \dot{\OO}^{\alpha'\beta'}(r_{2},\theta_{2})\Big)\Bigg) \, . \label{eq-null-z11-dd-int-6}
\end{align}
Now we need to write this as a (angular ordered) correlation function. To do this, we split the integrals for $\theta_{1}>\theta_{2}$ and for $\theta_{2}>\theta_{1}$. We get
\begin{align}
    \ddot{Z}_{n}^{(1,1)}& \, = \,\,  \sum_{\alpha'\beta'}\sum_{\alpha\beta} \, \int dr_{1}dr_{2} \, \int_{\theta_{1}>\theta_{2}} d\theta_{1}d\theta_{2} \,\, \tf_{\alpha\beta}(r_{1},\theta_{1}) \, \tf_{\alpha'\beta'}(r_{2},\theta_{2}) \,\,  \int_{-\infty}^{\infty} d\omega \, F_{n}(\omega) \nonumber\\ &\times  
    \Bigg( \tr \Big( \trho^{(0)} \, {\OO}_{\omega}^{\alpha\beta}(r_{1},\theta_{1}) \, \ddot{\OO}^{\alpha'\beta'}(r_{2},\theta_{2})\Big) + \, \tr \Big( \trho^{(0)} \, \dot{\OO}_{\omega}^{\alpha\beta}(r_{1},\theta_{1}) \, \dot{\OO}^{\alpha'\beta'}(r_{2},\theta_{2})\Big)\Bigg) \, \nonumber\\
    & \, + \,\, \sum_{\alpha'\beta'}\sum_{\alpha\beta} \, \int dr_{1}dr_{2} \, \int_{\theta_{1}<\theta_{2}} d\theta_{1}d\theta_{2} \,\, \tf_{\alpha\beta}(r_{1},\theta_{1}) \, \tf_{\alpha'\beta'}(r_{2},\theta_{2}) \,\,  \int_{-\infty}^{\infty} d\omega \, F_{n}(\omega) \, e^{-2\pi\omega} \nonumber\\ &\times  
    \Bigg( \tr \Big( \trho^{(0)}  \, \ddot{\OO}^{\alpha'\beta'}(r_{2},\theta_{2}) \, {\OO}_{\omega}^{\alpha\beta}(r_{1},\theta_{1})\Big) + \, \tr \Big( \trho^{(0)}  \, \dot{\OO}^{\alpha'\beta'}(r_{2},\theta_{2}) \, \dot{\OO}_{\omega}^{\alpha\beta}(r_{1},\theta_{1})\Big)\Bigg) \, ,\label{eq-null-z11-dd-int-7}
\end{align}
where we have used the commutation relation in Eq.~\eqref{eq-null-OOw-commutation} in the integral for $\theta_{1}<\theta_{2}$. 

Now using Eq.~\eqref{eq-null-Fn-def}, we note that
\begin{align}
    F_{n}(-x) \, = \, e^{-2\pi x} \, F_{n}(x) \, . \label{eq-null-F-x}
\end{align}
With this observation, we write Eq.~\eqref{eq-null-z11-dd-int-7} as
\begin{align}
     \ddot{Z}_{n}^{(1,1)} \, = \,&\,  \sum_{\alpha'\beta'}\sum_{\alpha\beta} \, \int dr_{1}dr_{2} \, \int_{0}^{2\pi} d\theta_{1}d\theta_{2} \,\, \tf_{\alpha\beta}(r_{1},\theta_{1}) \, \tf_{\alpha'\beta'}(r_{2},\theta_{2})  \nonumber\\ &\times \,  \int_{-\infty}^{\infty} d\omega \, F_{n}\Big(\text{sgn}(\theta_{1}-\theta_{2}) \, \omega\Big)  
    G_{\omega}\big(r_{1},r_{2},\theta_{1},\theta_{2} \, ; \alpha\beta\alpha'\beta'\big) \, , \label{eq-null-z11-corr}
\end{align}
where we have defined
\begin{align}
    G_{\omega}\big(r_{1},r_{2},\theta_{1},\theta_{2} \, ; \alpha\beta\alpha'\beta'\big) \, \equiv \, \left\langle {\OO}_{\omega}^{\alpha\beta}(r_{1},\theta_{1}) \, \ddot{\OO}^{\alpha'\beta'}(r_{2},\theta_{2}) \right\rangle \, + \, \Big\langle \dot{\OO}_{\omega}^{\alpha\beta}(r_{1},\theta_{1}) \, \dot{\OO}^{\alpha'\beta'}(r_{2},\theta_{2}) \Big\rangle \, . \label{eq-null-Gw-def}
\end{align}

To summarize this section, we have derived a formula for $\ddot{Z}_{n}^{(1,1)}$ in terms of a correlation functions. In the next sections, we will calculate $G_{\omega}$ in Eq.~\eqref{eq-null-Gw-def} and will use it in Sec.~(\ref{sec-proof-Renyi-QNEC}) to show that $\ddot{Z}_{n}^{(1,1)}$ in Eq.~\eqref{eq-null-z11-corr} is non-negative. This will prove the Renyi QNEC as discussed in Sec.~(\ref{sec-null-QNEC-stat}). 


\subsection{Proving the Renyi QNEC for $n>1$} \label{sec-proof-Renyi-QNEC}

We now insert $G_{\omega}$ from Eq.~\eqref{eq-null-Gs-final} in Eq.~\eqref{eq-null-z11-corr} to get
\begin{align}
    \ddot{Z}_{n}^{(1,1)} \, = \,&\,  \sum_{\alpha\beta} \, \int dr_{1}dr_{2} \, \int_{0}^{2\pi} d\theta_{1}d\theta_{2} \,\, \tf_{\alpha\beta}(r_{1},\theta_{1}) \, \tf_{\beta\alpha}(r_{2},\theta_{2}) \, e^{-2\pi K_{\alpha}} \,  \left(\frac{r_{1}}{r_{2}}\right)^{iv_{\alpha\beta}} \,  \nonumber\\ &\times \,  \frac{1}{ \, \big(r_{1} e^{i\theta_{1}}\big)^{2} \, \big(r_{2} e^{i\theta_{2}}\big)^{2}} \, \int_{-\infty}^{\infty} d\omega \, F_{n}\Big(\text{sgn}(\theta_{1}-\theta_{2}) \, \omega\Big)  
    \, \frac{H_{\omega}(\theta_{1}-\theta_{2}) }{ 1 - e^{-2\pi(v_{\alpha\beta} - \omega) }  } \label{eq-null-qnec-int}\\ &\times \, \Bigg\{ M_{\alpha\beta}\big({r_{1}}/{r_{2}} \, , \, \theta_{1}-\theta_{2} \,  | \, \omega\big) \, - \, M_{\alpha\beta}\big({r_{1}}/{r_{2}} \, , \, \theta_{1}-\theta_{2} \,  | \, \omega+i\big) \Bigg\}  \, . \nonumber 
\end{align}
Now note that we can combine Eq.~\eqref{eq-null-F-x} and Eq.~\eqref{eq-null-hw-def} to write
\begin{align}
    F_{n}\Big(\text{sgn}(\theta_{1}-\theta_{2}) \, \omega\Big) \, = \, F\big(\omega\big) \, \Big(  H_{\omega}(\theta_{1}-\theta_{2}) \Big)^{-1} \, .
\end{align}
With this result, Eq.~\eqref{eq-null-qnec-int} becomes
\begin{align}
    \ddot{Z}_{n}^{(1,1)} \, = \,&\,  \sum_{\alpha\beta} \, \int dr_{1}dr_{2} \, \int_{0}^{2\pi} d\theta_{1}d\theta_{2} \,\, \tf_{\alpha\beta}(r_{1},\theta_{1}) \, \tf_{\beta\alpha}(r_{2},\theta_{2}) \, e^{-2\pi K_{\alpha}} \,  \left(\frac{r_{1}}{r_{2}}\right)^{iv_{\alpha\beta}} \,  \nonumber\\ &\times \,  \frac{1}{ \, \big(r_{1} e^{i\theta_{1}}\big)^{2} \, \big(r_{2} e^{i\theta_{2}}\big)^{2}} \, \int_{-\infty}^{\infty} d\omega \, F_{n}\big(\omega\big)  
    \, \frac{1}{ 1 - e^{-2\pi(v_{\alpha\beta} - \omega) }  } \label{eq-null-qnec-int2}\\ &\times \, \Bigg\{ M_{\alpha\beta}\big({r_{1}}/{r_{2}} \, , \, \theta_{1}-\theta_{2} \,  | \, \omega\big) \, - \, M_{\alpha\beta}\big({r_{1}}/{r_{2}} \, , \, \theta_{1}-\theta_{2} \,  | \, \omega+i\big) \Bigg\}  \, . \nonumber 
\end{align}
Interestingly, all the dependence on $\text{sgn}(\theta_{1}-\theta_{2})$ finally drops out. We simplify the above result and write it as
\begin{align}
    \ddot{Z}_{n}^{(1,1)} \, = \,\frac{1}{2} &\,  \sum_{\alpha\beta} \, \int dr_{1}dr_{2} \, \int_{0}^{2\pi} d\theta_{1}d\theta_{2} \,\, \tf_{\alpha\beta}(r_{1},\theta_{1}) \, \tf_{\beta\alpha}(r_{2},\theta_{2}) \, e^{-\pi \left(K_{\alpha}+K_{\beta}\right)}  \,  \nonumber\\ &\times \,  \left(\frac{r_{1}}{r_{2}}\right)^{iv_{\alpha\beta}} \, \frac{1}{ \, \big(r_{1} e^{i\theta_{1}}\big)^{2} \, \big(r_{2} e^{i\theta_{2}}\big)^{2}} \, \int_{-\infty}^{\infty} d\omega \, \tF_{n}\big(\omega\big)  
    \, \frac{1}{ \sinh\big(\pi(v_{\alpha\beta} - \omega)\big)  } \label{eq-null-qnec-int3}\\ &\times \, \Bigg\{ M_{\alpha\beta}\big({r_{1}}/{r_{2}} \, , \, \theta_{1}-\theta_{2} \,  | \, \omega\big) \, - \, M_{\alpha\beta}\big({r_{1}}/{r_{2}} \, , \, \theta_{1}-\theta_{2} \,  | \, \omega+i\big) \Bigg\}  \, , \nonumber 
\end{align}
where we have defined
\begin{align}
     \tF_{n}\big(\omega\big) \, \equiv& \,\, e^{-\pi\omega} \, F_{n}\big(\omega\big) \, . 
\end{align}
Using Eq.~\eqref{eq-null-Fn-def}, we get
\begin{align}
    \tF_{n}\big(\omega\big) \, = \, \frac{n}{n-1} \, \frac{ \sinh\Big( \pi \big(\frac{n-1}{n}\big) \omega \Big)}{ \sinh\big(\pi \omega/n\big)} \, . \label{eq-null-tFn-def}
\end{align}

Note that so far we have taken $n$ to be arbitrary. From now on, we will assume that $n>1$. To simplify Eq.~\eqref{eq-null-qnec-int3}, consider the following integral over closed contour:
\begin{align}
    J_{\alpha\beta}\big({r_{1}}/{r_{2}} \, , \, \theta_{1}-\theta_{2} \big) \, \equiv \, \oint_{C} \, d\omega \, \frac{ \tF_{n}\big(\omega \, - \, i\big) }{\sinh\big(\pi(v_{\alpha\beta} - \omega)\big)} \, M_{\alpha\beta}\big({r_{1}}/{r_{2}} \, , \, \theta_{1}-\theta_{2} \,  | \, \omega\big)  \, , \label{eq-null-Jab-def}
\end{align}
where $C$ is an infinite rectangular contour:
\begin{align}
    C \, : \,\, (-\infty \, , \, \infty) \, \cup \, (\infty \, , \, \infty+i) \, \cup \, (\infty+i \, , \, -\infty+i) \, \cup \, (-\infty+i \, , \, -\infty) \,  .
\end{align}
Note that there are no poles (for $n>1$) of the integrand of Eq.~\eqref{eq-null-Jab-def} inside the contour $C$. Therefore, we get
\begin{align}
    J_{\alpha\beta}\big({r_{1}}/{r_{2}} \, , \, \theta_{1}-\theta_{2} \big) \, = \, 0 \, . \label{eq-null-Jab-zero}
\end{align}
Also, note that the integrand of Eq.~\eqref{eq-null-Jab-def} along the vertical contours at $\text{Re}(\omega) \, = \, \pm\infty$ vanishes. Therefore, only the integral along the horizontal contour contribute to the contour integral in Eq.~\eqref{eq-null-Jab-def}. This observation together with Eq.~\eqref{eq-null-Jab-zero} imply
\begin{align}
    0 \, =& \, \int_{-\infty}^{\infty} \, d\omega \, \frac{ \tF_{n}\big(\omega \, - \, i\big) }{\sinh\big(\pi(v_{\alpha\beta} - \omega)\big)} \, M_{\alpha\beta}\big({r_{1}}/{r_{2}} \, , \, \theta_{1}-\theta_{2} \,  | \, \omega\big)  \, \nonumber\\
    -& \, \int_{-\infty+i}^{\infty+i} \, d\omega \, \frac{ \tF_{n}\big(\omega \, - \, i\big) }{\sinh\big(\pi(v_{\alpha\beta} - \omega)\big)} \, M_{\alpha\beta}\big({r_{1}}/{r_{2}} \, , \, \theta_{1}-\theta_{2} \,  | \, \omega\big)  \, .
\end{align}
In other words,
\begin{align}
    0 \, =& \, \int_{-\infty}^{\infty} \, d\omega \, \frac{ \tF_{n}\big(\omega \, - \, i\big) }{\sinh\big(\pi(v_{\alpha\beta} - \omega)\big)} \, M_{\alpha\beta}\big({r_{1}}/{r_{2}} \, , \, \theta_{1}-\theta_{2} \,  | \, \omega\big)  \, \nonumber\\
    +& \, \int_{-\infty}^{\infty} \, d\omega \, \frac{ \tF_{n}\big(\omega \big) }{\sinh\big(\pi(v_{\alpha\beta} - \omega)\big)} \, M_{\alpha\beta}\big({r_{1}}/{r_{2}} \, , \, \theta_{1}-\theta_{2} \,  | \, \omega + i \big)  \, .\label{eq-null-int-rel}
\end{align}

Now using Eq.~\eqref{eq-null-int-rel}, we write Eq.~\eqref{eq-null-qnec-int3} as 
\begin{align}
    \ddot{Z}_{n}^{(1,1)} \, = \,\frac{1}{2} &\,  \sum_{\alpha\beta} \, \int dr_{1}dr_{2} \, \int_{0}^{2\pi} d\theta_{1}d\theta_{2} \,\, \tf_{\alpha\beta}(r_{1},\theta_{1}) \, \tf_{\beta\alpha}(r_{2},\theta_{2}) \, e^{-\pi \left(K_{\alpha}+K_{\beta}\right)}  \,  \nonumber\\ &\times \,  \left(\frac{r_{1}}{r_{2}}\right)^{iv_{\alpha\beta}} \, \frac{1}{ \, \big(r_{1} e^{i\theta_{1}}\big)^{2} \, \big(r_{2} e^{i\theta_{2}}\big)^{2}} \, \int_{-\infty}^{\infty} d\omega \, \Big( \tF_{n}\big(\omega\big) \, + \, \tF_{n}\big(\omega-i\big) \Big)  
    \,  \label{eq-null-qnec-int4}\\ &\times \, \frac{1}{ \sinh\big(\pi(v_{\alpha\beta} - \omega)\big)  } \,  M_{\alpha\beta}\big({r_{1}}/{r_{2}} \, , \, \theta_{1}-\theta_{2} \,  | \, \omega\big) \,  . \nonumber 
\end{align}
Now we use Eq.~\eqref{eq-null-Mab-def} and get
\begin{align}
    \ddot{Z}_{n}^{(1,1)} \, = \,\frac{1}{2} &\,  \sum_{\alpha\beta} \, e^{-\pi \left(K_{\alpha}+K_{\beta}\right)}  \,  \int_{-\infty}^{\infty} d\omega \, \Big( \tF_{n}\big(\omega\big) \, + \, \tF_{n}\big(\omega-i\big) \Big)  \, \frac{(v_{\alpha\beta} - \omega)\left((v_{\alpha\beta} - \omega)^{2}+1\right)}{ \sinh\big(\pi(v_{\alpha\beta} - \omega)\big)  } \nonumber\\
    &\times \, \int dr_{1} \, \int_{0}^{2\pi} d\theta_{1}\, \tf_{\alpha\beta}(r_{1},\theta_{1}) \, \left(r_{1}\right)^{iv_{\alpha\beta}-i\omega-2} \, e^{-(2i-\omega)\theta_{1}} \label{eq-null-qnec-int5}\\ 
    &\times \, \int dr_{2} \, \int_{0}^{2\pi} d\theta_{2}\, \tf_{\beta\alpha}(r_{2},\theta_{2}) \, \left(r_{2}\right)^{-iv_{\alpha\beta}+i\omega-2} \, e^{-(2i+\omega)\theta_{2}}\,  . \nonumber 
\end{align}
%\begin{align}
 %   \ddot{Z}_{n}^{(1,1)} \, = \,\frac{1}{2} &\,  \sum_{\alpha\beta} \, e^{-\pi \left(K_{\alpha}+K_{\beta}\right)}  \,  \int_{-\infty}^{\infty} d\omega \, \Big( \tF_{n}\big(\omega\big) \, + \, \tF_{n}\big(\omega-i\big) \Big)  \, \frac{(v_{\alpha\beta} - \omega)\left((v_{\alpha\beta} - \omega)^{2}+1\right)}{ \sinh\big(\pi(v_{\alpha\beta} - \omega)\big)  } \nonumber\\
  %  &\times \, \int dr_{1}dr_{2} \, \int_{0}^{2\pi} d\theta_{1}d\theta_{2} \,\, \tf_{\alpha\beta}(r_{1},\theta_{1}) \, \tf_{\beta\alpha}(r_{2},\theta_{2}) \,   \label{eq-null-qnec-int5}\\ &\times \,\left(\frac{r_{1}}{r_{2}}\right)^{iv_{\alpha\beta}-i\omega} \, \frac{1}{ \, \big(r_{1} e^{i\theta_{1}}\big)^{2} \, \big(r_{2} e^{i\theta_{2}}\big)^{2}} \, e^{\omega(\theta_{1}-\theta_{2})}  \,  . \nonumber 
%\end{align}

Now note that we are free to take $\alpha \leftrightarrow \beta$, $(r_{1},\theta_{1}) \leftrightarrow (r_{2},\theta_{2})$, and $\omega \to -\omega$ in Eq.~\eqref{eq-null-qnec-int5}. Under this change of dummy variables, Eq.~\eqref{eq-null-qnec-int5} becomes
\begin{align}
    \ddot{Z}_{n}^{(1,1)} \, = \,\frac{1}{2} &\,  \sum_{\alpha\beta} \, e^{-\pi \left(K_{\alpha}+K_{\beta}\right)}  \,  \int_{-\infty}^{\infty} d\omega \, \Big( \tF_{n}\big(\omega\big) \, + \, \tF_{n}\big(\omega+i\big) \Big)  \, \frac{(v_{\alpha\beta} - \omega)\left((v_{\alpha\beta} - \omega)^{2}+1\right)}{ \sinh\big(\pi(v_{\alpha\beta} - \omega)\big)  } \nonumber\\
    &\times \, \int dr_{1} \, \int_{0}^{2\pi} d\theta_{1}\, \tf_{\alpha\beta}(r_{1},\theta_{1}) \, \left(r_{1}\right)^{iv_{\alpha\beta}-i\omega-2} \, e^{-(2i-\omega)\theta_{1}} \label{eq-null-qnec-int6}\\ 
    &\times \, \int dr_{2} \, \int_{0}^{2\pi} d\theta_{2}\, \tf_{\beta\alpha}(r_{2},\theta_{2}) \, \left(r_{2}\right)^{-iv_{\alpha\beta}+i\omega-2} \, e^{-(2i+\omega)\theta_{2}}\,  . \nonumber 
\end{align}
We combine Eq.~\eqref{eq-null-qnec-int5} and Eq.~\eqref{eq-null-qnec-int6} to get
\begin{align}
    \ddot{Z}_{n}^{(1,1)} \, = \,\frac{1}{4} &\,  \sum_{\alpha\beta} \, e^{-\pi \left(K_{\alpha}+K_{\beta}\right)}  \,  \int_{-\infty}^{\infty} d\omega \, \Big( 2\tF_{n}\big(\omega\big) \, + \, \tF_{n}\big(\omega+i\big) \, + \, \tF_{n}\big(\omega-i\big) \Big) \, Q(v_{\alpha\beta} - \omega) \nonumber\\
    &\times \, \int dr_{1} \, \int_{0}^{2\pi} d\theta_{1}\, \tf_{\alpha\beta}(r_{1},\theta_{1}) \, \left(r_{1}\right)^{iv_{\alpha\beta}-i\omega-2} \, e^{-(2i-\omega)\theta_{1}} \label{eq-null-qnec-int7}\\ 
    &\times \, \int dr_{2} \, \int_{0}^{2\pi} d\theta_{2}\, \tf_{\beta\alpha}(r_{2},\theta_{2}) \, \left(r_{2}\right)^{-iv_{\alpha\beta}+i\omega-2} \, e^{-(2i+\omega)\theta_{2}}\,  , \nonumber 
\end{align}
where we have defined
\begin{align}
    Q(x) \, \equiv \, \frac{x(x^{2}+1)}{\sinh (\pi x)} \, .
\end{align}
Finally, we take $\theta_{2} \to (2\pi-\theta_{2})$ and use the reality condition in Eq.~\eqref{eq-null-reality} to get
\begin{align}
    \ddot{Z}_{n}^{(1,1)} \, = \,&\frac{1}{4} \,  \sum_{\alpha\beta} \, e^{-\pi \left(K_{\alpha}+K_{\beta}\right)}  \,  \int_{-\infty}^{\infty} d\omega \, \Big( 2\tF_{n}\big(\omega\big) \, + \, \tF_{n}\big(\omega+i\big) \, + \, \tF_{n}\big(\omega-i\big) \Big) \,  \nonumber\\
    &\times \, e^{2\pi\omega} \, Q(v_{\alpha\beta} - \omega) \, \Bigg|\int dr \, \int_{0}^{2\pi} d\theta\, \tf_{\alpha\beta}(r,\theta) \, r^{iv_{\alpha\beta}-i\omega-2} \, e^{-(2i-\omega)\theta}\Bigg|^{2} \, . \label{eq-null-qnec-fin}
\end{align}
The second line in Eq.~\eqref{eq-null-qnec-fin} is non-negative. Therefore, to prove the Renyi QNEC (for $n>1$), we need to show that the first line in Eq.~\eqref{eq-null-qnec-fin} is also non-negative. We deduce from Eq.~\eqref{eq-null-tFn-def} that %$\tF_{n}\big(\omega\big) \ge 0$. Moreover, we deduce from  Eq.~\eqref{eq-null-tFn-def} that
\begin{align}
    2\tF_{n}\big(\omega\big) \, + \, \tF_{n}\big(\omega+i\big) \, + \, \tF_{n}\big(\omega-i\big) \, = \, \frac{2n}{n-1} \, \frac{\sinh(\pi\omega)}{\tanh\big(\pi\omega/n\big)} \, \frac{\sin^{2}\big(\pi/n\big)}{\sinh^{2}\big(\pi\omega/n\big)+\sin^{2}\big(\pi/n\big)} \, ,\label{eq-null-fnw-final}
\end{align}
which is non-negative for $n>1$. Hence, we deduce from Eq.~\eqref{eq-null-qnec-fin} that
\begin{align}
    \ddot{Z}_{n}^{(1,1)} \, \ge \, 0 \, .
\end{align}
This finishes our proof of the Renyi QNEC for all $n>1$. 

\subsection{Recovering the known result for $n=1$}

In this section, our goal is to take $n\to 1$ limit of our result in Eq.~\eqref{eq-null-qnec-fin} and to recover the result of \cite{Bousso:2015wca}. To do this, we need to take $n \to 1$ limit of Eq.~\eqref{eq-null-fnw-final}. 

We start by defining:
\begin{align}
    \widehat{F}_{1}\big(\omega\big) \, \equiv \lim_{n\to 1} \, \Big[ 2\tF_{n}\big(\omega\big) \, + \, \tF_{n}\big(\omega+i\big) \, + \, \tF_{n}\big(\omega-i\big) \Big] \, .
\end{align}
Using Eq.~\eqref{eq-null-fnw-final}, we get
\begin{align}
    \widehat{F}_{1}\big(\omega\big) \, = \, \frac{2 \, \sinh(\pi\omega)}{\tanh\big(\pi\omega\big)} \, \lim_{n \to 1} \, \left[ \frac{1}{n-1} \, \frac{\sin^{2}\big(\pi/n\big)}{\sinh^{2}\big(\pi\omega/n\big)+\sin^{2}\big(\pi/n\big)} \right] \, . \label{eq-null-fnw-lim-1}
\end{align}
Now note that near $n = 1$,
\begin{align}
    \sin^{2}(\pi/n) \, = \, \pi^{2} \, (n-1)^{2} \, + O\Big( (n-1)^{3} \Big) \, . 
\end{align}
Using this result, Eq.~\eqref{eq-null-fnw-lim-1} becomes
\begin{align}
    \widehat{F}_{1}\big(\omega\big) \, = \, \frac{2 \, \sinh(\pi\omega)}{\tanh\big(\pi\omega\big)} \, \lim_{n \to 1} \, \left[  \frac{(n-1)}{(n-1)^{2} \, + \, \pi^{-2} \, \sinh^{2}\big(\pi\omega\big)} \right] \, . \label{eq-null-fnw-lim-2}
\end{align}
Now recall the identity
\begin{align}
    \delta(x) \, = \, \lim_{\epsilon\to 0} \, \frac{1}{\pi} \, \frac{\epsilon}{\epsilon^{2}+x^{2}} \, .
\end{align}
With this identity, Eq.~\eqref{eq-null-fnw-lim-2} reduces to 
\begin{align}
    \widehat{F}_{1}\big(\omega\big) \, = \, 2\pi \, \delta\big(\omega\big)  \, . \label{eq-null-fnw-lim-3}
\end{align}

Therefore, the limit $n\to 1$ of Eq.~\eqref{eq-null-qnec-fin} is
\begin{align}
    \lim_{n\to 1} \, \ddot{Z}_{n}^{(1,1)} \, = \, \frac{\pi}{2} \,  \sum_{\alpha\beta} \, e^{-\pi \left(K_{\alpha}+K_{\beta}\right)}  \,  Q(v_{\alpha\beta}) \, \Bigg|\int dr \, \int_{0}^{2\pi} d\theta\, \tf_{\alpha\beta}(r,\theta) \, r^{iv_{\alpha\beta}-2} \, e^{-2i\theta}\Bigg|^{2} \, .
\end{align}
This precisely matches the known result from \cite{Bousso:2015wca} (also see \cite{Balakrishnan:2019gxl}).
